On the Inefficiency of Forward Markets in Leader-Follower Competition

Motivated by electricity markets, this paper studies the impact of forward contracting in situations where firms have capacity constraints and heterogeneous production lead times. We consider a model with two types of firms - leaders and followers - that choose production at two different times. Followers choose productions in the second stage but can sell forward contracts in the first stage. Our main result is an explicit characterization of the equilibrium outcomes. Classic results on forward contracting suggest that it can mitigate market power in simple settings; however the results in this paper show that the impact of forward markets in this setting is delicate - forward contracting can enhance or mitigate market power. In particular, our results show that leader-follower interactions created by heterogeneous production lead times may cause forward markets to be inefficient, even when there are a large number of followers. In fact, symmetric equilibria do not necessarily exist due to differences in market power among the leaders and followers.

==> summary.tex <==
\section{Summary of Main Insights}
\label{sec:MainResults}

\adam{This section needs work -- the conclusion does a better job of making the results sound exciting at this point...Let's talk about this.}

Our model differs from previous studies on forward contracting in two important aspects. First, in our model, firms may choose productions (not just forward contracts) in the forward market, which is a feature that has not been investigated before. Second, in our model, firms have capacity constraints, while the majority of forward market studies, with the exception of~\cite{murphy2010impact,kamat2004two}, assume unconstrained productions. Our results provide two macro insights into the strategic interactions created by these features.

Our first insight is that forward contracting may decrease the efficiency of the market. The reason is that forward contracting may create opportunities for leaders to exploit the capacity constraints of followers. Conventional intuition on the prisoner's dilemma effect of forward contracting suggests that followers should increase their productions, e.g., as in~\cite{allaz1993cournot}. However, this may cause followers to operate closer to capacity. Leaders, in order to exploit the fact that followers are now \emph{less flexible}, may reduce their productions to the extent that the equilibrium total market production decreases. Informally, the increased competition due to forward contracting is offset by the decreased competition faced by the leaders due to followers being capacity constrained. Hence, the capacity constraints create opportunities for market manipulation. Note that, while~\cite{murphy2010impact} also showed that forward contracting may decrease the efficiency of the market, theirs was a different phenomenon caused by the impact of forward contracting on capacity investment.

\adam{This needs to start with a more punchy sentence} Our second insight is that non-existence of symmetric equilibria can be attributed to exploitation of capacity constraints. The reason is that each firm's individual incentive to exploit the capacity constraints of followers could lead to disequilibrium in the forward market. When any follower operates close to capacity, other firms have a strategic incentive to exploit the fact that this follower is now \emph{less flexible} by reducing their forward positions. However, if all firms were to reduce their forward positions simultaneously, the high prices would create incentives for them to increase their forward positions. Therefore, there is no symmetric equilibrium. While~\cite{murphy2010impact} also observed that equilibria may not exist when there are capacity constraints, their argument was based on showing that profit functions are not convex and no explicit conditions or strategic insights were provided. In contrast, we give explicit conditions under which symmetric equilibria do not exist and hence are able to explain how strategic withholding precludes symmetric equilibrium.


